The two-user Gaussian interference channel: a deterministic view

This paper explores the two-user Gaussian interference channel through the lens of a natural deterministic channel model. The main result is that the deterministic channel uniformly approximates the Gaussian channel, the capacity regions differing by a universal constant. The problem of finding the capacity of the Gaussian channel to within a constant error is therefore reduced to that of finding the capacity of the far simpler deterministic channel. Thus, the paper provides an alternative derivation of the recent constant gap capacity characterization of Etkin, Tse, and Wang. Additionally, the deterministic model gives significant insight towards the Gaussian channel.

==> Fig_universalApproximation.tex <==
\psset{unit=1.2mm,linewidth=.3pt,arrowlength=1.2,
arrowinset=0,labelsep=3pt}
\begin{center}
\begin{pspicture}(0,2)(40,25)
\psline{->}(0,0)(40,0)
\psline{->}(0,0)(0,20)

\uput[l](0,20){\scriptsize $\snr_2$}
\uput[d](40,0){\scriptsize $\snr_1$}

\pscurve(3,0)(10,6)(18,4)(25,8)(40,11)
\uput[u](10,6){$f$}

\end{pspicture}
\end{center} 
